Prompt-In-Prompt Learning for Universal Image Restoration

Image restoration, which aims to retrieve and enhance degraded images, is fundamental across a wide range of applications. While conventional deep learning approaches have notably improved the image quality across various tasks, they still suffer from (i) the high storage cost needed for various task-specific models and (ii) the lack of interactivity and flexibility, hindering their wider application. Drawing inspiration from the pronounced success of prompts in both linguistic and visual domains, we propose novel Prompt-In-Prompt learning for universal image restoration, named PIP. First, we present two novel prompts, a degradation-aware prompt to encode high-level degradation knowledge and a basic restoration prompt to provide essential low-level information. Second, we devise a novel prompt-to-prompt interaction module to fuse these two prompts into a universal restoration prompt. Third, we introduce a selective prompt-to-feature interaction module to modulate the degradation-related feature. By doing so, the resultant PIP works as a plug-and-play module to enhance existing restoration models for universal image restoration. Extensive experimental results demonstrate the superior performance of PIP on multiple restoration tasks, including image denoising, deraining, dehazing, deblurring, and low-light enhancement. Remarkably, PIP is interpretable, flexible, efficient, and easy-to-use, showing promising potential for real-world applications. The code is available at https://github.com/longzilicart/pip_universal.

==> sec/5._discussion.tex <==



==> tab/compare_single.tex <==
\begin{table*}[htb]
    \centering
    \caption{Denoising comparisons in the single-task setting on BSD68 and Urban100 datasets.}
    \label{tab:denoising}
    \small
    \resizebox{\textwidth}{!}{
    \begin{tabular}{@{}c|cccc|cccc@{}}
        \toprule
        \multicolumn{5}{c|}{BSD68} & \multicolumn{4}{c}{Urban100} \\
        Method & $\sigma = 15$ & $\sigma = 25$ & $\sigma = 50$ & Average & $\sigma = 15$ & $\sigma = 25$ & $\sigma = 50$ & Average \\
        \midrule
        CBM3D & 33.50/0.922 & 30.69/0.868 & 27.36/0.763 & - & 33.93/0.941 & 31.36/0.909 & 27.93/0.840 & - \\
        DnCNN & 33.89/0.930 & 31.23/0.883 & 27.92/0.789 & - & 32.98/0.931 & 30.81/0.902 &  27.59/0.833 & - \\
        IRCNN & 33.87/0.929 & 31.18/0.882 &  27.88/0.790 & - & 27.59/0.833 & 31.20/0.909 & 27.70/0.840 & - \\
        FFDNet & 33.87/0.929 & 31.21/0.882 & 27.96/0.789 & - & 33.83/0.942 &  31.40/0.912 & 28.05/0.848 & - \\
        BRDNet & 34.10/0.929 & 31.43/0.885 &  28.16/0.794 & - & 34.42/0.946 & 31.99/0.919 & 28.56/0.858 & - \\
        AirNet & 34.14/0.936 &  31.48/0.893 & 28.23/0.806 & - & 34.40/0.949 & 32.10/0.924 & 28.88/0.871 & - \\
        Restormer & 34.29/0.937 & 31.64/0.895 & 28.41/0.810 & - & 34.67/0.969 & 32.41/0.927 & 29.31/0.878 & - \\
        % \rowcolor{Gray}
        PromptIR(Ours) & 34.34/0.938 & 31.71/0.897 & 28.49/0.813 & - & 34.77/0.952 & 32.49/0.929 & 29.39/0.881 & - \\
        \midrule
        \methodname & - & - & - & - & - & - & - & - \\
        \bottomrule
      \end{tabular}}
    \end{table*}

